Contextual Predictive Mutation Testing

Mutation testing is a powerful technique for assessing and improving test suite quality that artificially introduces bugs and checks whether the test suites catch them. However, it is also computationally expensive and thus does not scale to large systems and projects. One promising recent approach to tackling this scalability problem uses machine learning to predict whether the tests will detect the synthetic bugs, without actually running those tests. However, existing predictive mutation testing approaches still misclassify 33% of detection outcomes on a randomly sampled set of mutant-test suite pairs. We introduce MutationBERT, an approach for predictive mutation testing that simultaneously encodes the source method mutation and test method, capturing key context in the input representation. Thanks to its higher precision, MutationBERT saves 33% of the time spent by a prior approach on checking/verifying live mutants. MutationBERT, also outperforms the state-of-the-art in both same project and cross project settings, with meaningful improvements in precision, recall, and F1 score. We validate our input representation, and aggregation approaches for lifting predictions from the test matrix level to the test suite level, finding similar improvements in performance. MutationBERT not only enhances the state-of-the-art in predictive mutation testing, but also presents practical benefits for real-world applications, both in saving developer time and finding hard to detect mutants.

==> Makefile <==
# Set this to the basename of the .tex file
# This will also be the name of the generated .dvi, .ps and .pdf files

.PHONY: original revised diff all clean

# Set this to the other source files that should be counted as
# dependencies
OTHERSOURCES := bibliography.bib \
	acmart.bib
#	$(filter-out $DOC, $(wildcard *.tex))

all: main

original: fse.pdf
	mv fse.pdf original.pdf

main: main.pdf

diff: main.tex main.pdf
	mv main.pdf diff.pdf

tidy:
	rm -rf *.aux *.out *.bbl *.toc *.log *.blg *.pyg *.cpt _minted*

# Using latexmk to generate the PDF
%.pdf: %.tex $(OTHERSOURCES)
	latexmk -pdf -pdflatex="pdflatex -interaction=nonstopmode" -use-make $<

clean: tidy
	latexmk -CA

